TReC: Evaluating Move-Induced State Changes in Instruction-Conditioned Go

When a Go model predicts a move different from the expert's, coordinate distance measures how far the prediction lands from the reference. We introduce Transition Representation Consistency (TReC) to compare how the two moves change a board-state embedding. Both moves are executed from the same position under the game rules, and TReC is the cosine similarity between the two resulting representation changes. In experiments with a frozen KataGo network on 680 mid-to-late-game positions from five games, the gap between the highest and lowest candidate per position has a median of 0.01 to 0.08 for the direct successor-state cosine and 0.88 to 1.33 for TReC, depending on the evaluator layer. TReC follows coordinate distance only weakly: the rank correlation between a candidate's distance to the reference and its TReC, computed within each position, has a median of -0.19 over these positions.

==> preprint/frontmatter.tex <==
% Keep author contribution and correspondence notes below affiliations.
\makeatletter
\newcommand{\affiliations}[1]{\gdef\TrecAffiliations{#1}}
\newcommand{\equalcontrib}{\textsuperscript{*}}
\gdef\TrecContactNote{}
\renewcommand{\maketitle}{%
  \thispagestyle{plain}
  \begingroup
  \renewcommand{\thanks}[1]{\textsuperscript{\ensuremath{\dagger}}\gdef\TrecContactNote{##1}}
  \setlength{\parindent}{0pt}
  {\fontsize{21}{25}\selectfont\bfseries\color{TrecInk}\@title\par}
  \vspace{14pt}
  {\fontsize{11.5}{15}\selectfont\@author\par}
  \vspace{7pt}
  {\fontsize{9}{11.5}\selectfont\color{TrecMuted}\TrecAffiliations\par}
  \vspace{7pt}
  {\fontsize{8.5}{11}\selectfont\color{TrecMuted}%
    \textsuperscript{*}These authors contributed equally.\quad
    \textsuperscript{\ensuremath{\dagger}}\TrecContactNote\par}
  \vspace{13pt}
  {\color{TrecRule}\hrule height .6pt}
  \vspace{12pt}
  \endgroup
}
\renewenvironment{abstract}
  {\begingroup\setlength{\parindent}{0pt}\small
   \noindent{\sffamily\bfseries\color{TrecInk}Abstract}\par\nobreak\vspace{4pt}\noindent}
  {\par\vspace{10pt}{\color{TrecRule}\hrule height .6pt}\vspace{4pt}\endgroup}
\makeatother

